Analyzing Social Media Engagement of Computer Science Conferences

Context: X, formerly known as Twitter, is one of the largest social media platforms and has been widely used for communication during research conferences. While previous studies have examined how users engage with X during these events, limited research has focused on analyzing the content posted by computer science conferences. Objective: This study investigates how conferences from different areas of computer science perform on social media by analyzing their activity, follower engagement, and the content posted on X. Method: We collect posts from 22 computer science conferences and conduct statistical experiments to identify variations in content. Additionally, we perform a manual analysis of the top five posts for each engagement metric. Results: Our findings indicate statistically significant differences in category, sentiment, and post length across computer science conference posts. Among all engagement metrics, likes were the most common way users interacted with conference content. Conclusion: This study provides insights into the social media presence of computer science conferences, highlighting key differences in content, sentiment, and engagement patterns across different venues.

==> fig/table.tex <==
\begin{table}[]
\begin{tabular}{|l|l|l|l|l|}
\hline
Metric   & Tweet ID & Conference & Tweet Link                                                        & Metric Value \\ \hline
         & 241      & ICML       & https://twitter.com/icmlconf/status/1753410113325396168\#m        & 12           \\ \cline{2-5} 
         & 114      & CVPR       & https://twitter.com/CVPR/status/1712860756507861215\#m            & 8            \\ \cline{2-5} 
Comments & 271      & WSDM       & https://twitter.com/saiphcita/status/1753114041441288246\#m       & 7            \\ \cline{2-5} 
         & 379      & SIGACT     & https://twitter.com/sigact/status/1638906817219809280\#m          & 7            \\ \cline{2-5} 
         & 86       & IEEE       & https://twitter.com/kakbarihamed/status/1664748667272658945\#m    & 4            \\ \hline
         & 265      & ICML       & https://twitter.com/icmlconf/status/1683917606900858880\#m        & 269          \\ \cline{2-5} 
         & 242      & ICML       & https://twitter.com/zicokolter/status/1753398445216604588\#m      & 249          \\ \cline{2-5} 
Likes    & 259      & ICML       & https://twitter.com/icmlconf/status/1684634850492571652\#m        & 234          \\ \cline{2-5} 
         & 74       & IEEE       & https://twitter.com/ieee\_ras\_icra/status/1676953949998567424\#m & 189          \\ \cline{2-5} 
         & 302      & EMNLP      & https://twitter.com/emnlpmeeting/status/1733774582543458413\#m    & 172          \\ \hline
         & 138      & CVPR       & https://twitter.com/CVPR/status/1754905564906185162\#m            & 11           \\ \cline{2-5} 
         & 374      & SIGACT     & https://twitter.com/sigact/status/1659270972862775296\#m          & 10           \\ \cline{2-5} 
Quotes   & 379      & SIGACT     & https://twitter.com/sigact/status/1638906817219809280\#m          & 10           \\ \cline{2-5} 
         & 259      & ICML       & https://twitter.com/icmlconf/status/1684634850492571652\#m        & 9            \\ \cline{2-5} 
         & 265      & ICML       & https://twitter.com/icmlconf/status/1683917606900858880\#m        & 8            \\ \hline
         & 265      & ICML       & https://twitter.com/icmlconf/status/1683917606900858880\#m        & 59           \\ \cline{2-5} 
         & 259      & ICML       & https://twitter.com/icmlconf/status/1684634850492571652\#m        & 48           \\ \cline{2-5} 
Retweets & 242      & ICML       & https://twitter.com/zicokolter/status/1753398445216604588\#m      & 39           \\ \cline{2-5} 
         & 138      & CVPR       & https://twitter.com/CVPR/status/1754905564906185162\#m            & 31           \\ \cline{2-5} 
         & 205      & IEEESSP    & https://twitter.com/zsavvas90/status/1602967405612900354\#m       & 31           \\ \hline
\end{tabular}
\end{table}

==> tbl/complete_data_pvalue_correction_post_len.tex <==
\begin{table*}[htb]

\caption{Conference Post Hoc Test Complete Dataset P-Values}

\label{tbl_pvalues_complete}


\centering
% \renewcommand{\arraystretch}{1.25}
\resizebox{\linewidth}{!}{
\begin{tabular}{lllllllllllllllllllllll}
           & \rotatebox{90}{ASE} & \rotatebox{90}{CAV} & \rotatebox{90}{CVPR} & \rotatebox{90}{EC } & \rotatebox{90}{EMNLP} & \rotatebox{90}{EuroCrypt} & \rotatebox{90}{ICDE} & \rotatebox{90}{ICML} & \rotatebox{90}{ICRA} & \rotatebox{90}{IJCAI} & \rotatebox{90}{ISCA} & \rotatebox{90}{MobiCom} & \rotatebox{90}{NSDI} & \rotatebox{90}{Oakland} & \rotatebox{90}{PPoPP} & \rotatebox{90}{RTSS} & \rotatebox{90}{ {\tiny \textbf{SIGGRAPH}}} & \rotatebox{90}{{\tiny \textbf{SIGMETRICS}}} & \rotatebox{90}{SOSP} & \rotatebox{90}{Stoc}  & \rotatebox{90}{UIST} & \rotatebox{90}{WSDM}\\
        
ASE        & -   & **  & -    & *** & -     & ***       & ***  & ***  & -    & ***   & -    & *       & *    & ***     & -     & -    & ***      & ***        & -    & ***  & -    & ***  \\
CAV        & **  & -   & -    & *** & -     & ***       & ***  & -    & -    & -     & ***  & ***     & -    & -       & ***   & -    & ***      & ***        & -    & ***  & ***  & ***  \\
CVPR       & -   & -   & -    & *** & -     & ***       & ***  & ***  & -    & ***   & *    & ***     & -    & ***     & -     & -    & ***      & ***        & -    & ***  & -    & ***  \\
EC         & *** & *** & ***  & -   & ***   & ***       & ***  & **   & ***  & ***   & ***  & ***     & ***  & ***     & ***   & ***  & -        & -          & ***  & ***  & ***  & ***  \\
EMNLP      & -   & -   & -    & *** & -     & ***       & ***  & -    & -    & -     & ***  & ***     & -    & -       & *     & -    & ***      & ***        & -    & ***  & **   & ***  \\
EuroCrypt  & *** & *** & ***  & *** & ***   & -         & -    & ***  & ***  & ***   & -    & **      & ***  & ***     & -     & -    & ***      & ***        & **   & -    & ***  & -    \\
ICDE       & *** & *** & ***  & *** & ***   & -         & -    & ***  & ***  & ***   & -    & -       & ***  & ***     & -     & -    & ***      & ***        & -    & *    & **   & -    \\
ICML       & *** & -   & ***  & **  & -     & ***       & ***  & -    & ***  & *     & ***  & ***     & ***  & -       & ***   & ***  & ***      & ***        & **   & ***  & ***  & ***  \\
ICRA       & -   & -   & -    & *** & -     & ***       & ***  & ***  & -    & -     & ***  & ***     & -    & -       & *     & -    & ***      & ***        & -    & ***  & ***  & ***  \\
IJCAI      & *** & -   & ***  & *** & -     & ***       & ***  & *    & -    & -     & ***  & ***     & -    & -       & ***   & *    & ***      & ***        & -    & ***  & ***  & ***  \\
ISCA       & -   & *** & *    & *** & ***   & -         & -    & ***  & ***  & ***   & -    & -       & ***  & ***     & -     & -    & ***      & ***        & -    & ***  & -    & -    \\
MobiCom    & *   & *** & ***  & *** & ***   & **        & -    & ***  & ***  & ***   & -    & -       & ***  & ***     & -     & -    & ***      & ***        & -    & ***  & -    & ***  \\
NSDI       & *   & -   & -    & *** & -     & ***       & ***  & ***  & -    & -     & ***  & ***     & -    & -       & *     & -    & ***      & ***        & -    & ***  & ***  & ***  \\
Oakland    & *** & -   & ***  & *** & -     & ***       & ***  & -    & -    & -     & ***  & ***     & -    & -       & ***   & *    & ***      & ***        & -    & ***  & ***  & ***  \\
PPoPP      & -   & *** & -    & *** & *     & -         & -    & ***  & *    & ***   & -    & -       & *    & ***     & -     & -    & ***      & ***        & -    & -    & -    & -    \\
RTSS       & -   & -   & -    & *** & -     & -         & -    & ***  & -    & *     & -    & -       & -    & *       & -     & -    & ***      & ***        & -    & ***  & -    & -    \\
SIGGRAPH   & *** & *** & ***  & -   & ***   & ***       & ***  & ***  & ***  & ***   & ***  & ***     & ***  & ***     & ***   & ***  & -        & -          & ***  & ***  & ***  & ***  \\
SIGMETRICS & *** & *** & ***  & -   & ***   & ***       & ***  & ***  & ***  & ***   & ***  & ***     & ***  & ***     & ***   & ***  & -        & -          & ***  & ***  & ***  & ***  \\
SOSP       & -   & -   & -    & *** & -     & **        & -    & **   & -    & -     & -    & -       & -    & -       & -     & -    & ***      & ***        & -    & ***  & -    & ***  \\
Stoc       & *** & *** & ***  & *** & ***   & -         & *    & ***  & ***  & ***   & ***  & ***     & ***  & ***     & -     & ***  & ***      & ***        & ***  & -    & ***  & *    \\
UIST       & -   & *** & -    & *** & **    & ***       & **   & ***  & ***  & ***   & -    & -       & ***  & ***     & -     & -    & ***      & ***        & -    & ***  & -    & ***  \\
WSDM       & *** & *** & ***  & *** & ***   & -         & -    & ***  & ***  & ***   & -    & ***     & ***  & ***     & -     & -    & ***      & ***        & ***  & *    & ***  & -   
  
\end{tabular}
}
{
Here, $\ast$: p-value$ < $0.05 ,$\ast \ast$: p-value$ < $0.01
, and  $\ast \ast \ast$: p-value$ < $0.001
}
\end{table*}








==> tbl/tbl_top10_conf.tex <==
\begin{table}[htb]
\caption{Top 10 Conference}
\renewcommand{\arraystretch}{1.3}

\label{tbl_form_top10}

\begin{tabular}{|p{0.05\linewidth}|p{0.25\linewidth}|p{0.25\linewidth}|p{0.22\linewidth}|}
\hline
   & Twitter User    & Followers & Following \\ \hline
1  & icmlconf        & 74115     & 16        \\ \hline
2  & CVPR            & 44594     & 328       \\ \hline
3  & siggraph        & 43666     & 1734      \\ \hline
4  & usenix          & 14244     & 880       \\ \hline
5  & emnlpmeeting    & 13143     & 41        \\ \hline
6  & ieee\_ras\_icra & 10425     & 87        \\ \hline
7  & IEEESSP         & 9094      & 0         \\ \hline
8  & IJCAIconf       & 6776      & 831       \\ \hline
9  & ACMUIST         & 5302      & 67        \\ \hline
10 & WSDMSocial      & 3099      & 118       \\ \hline
\end{tabular}
\end{table}

==> tbl/tbl_top10_ratios.tex <==
\begin{table}[htb]
\caption{ Follower/Following Ratio, Retweet and Mention Ratio, Interactor Ratio and Klout score of each Conference}
\renewcommand{\arraystretch}{1.3}

\label{tbl_ratio_top10}

\begin{tabular}{|p{0.025\linewidth}|p{0.18\linewidth}|p{0.10\linewidth}|p{0.08\linewidth}|p{0.08\linewidth}|p{0.10\linewidth}|p{0.10\linewidth}|}
\hline
   & Twitter User    & FFr                    & RMi   & Ir    & RMi\_All & Ir\_All \\ \hline
1  & icmlconf        & 4632.2                 & 0.004 & 0.004 & 0.309    & 0.287   \\ \hline
2  & CVPR            & 136                    & 0.005 & 0.004 & 0.209    & 0.178   \\ \hline
3  & siggraph        & 25.182                 & 0.001 & 0.001 & 0.396    & 0.364   \\ \hline
4  & usenix          & 16.186                 & 0.002 & 0.002 & 0.165    & 0.135   \\ \hline
5  & emnlpmeeting    & 320.561                & 0.005 & 0.004 & 0.190    & 0.164   \\ \hline
6  & ieee\_ras\_icra & 119.828                & 0.027 & 0.024 & 0.547    & 0.504   \\ \hline
7  & IEEESSP         & \multicolumn{1}{c|}{-} & 0.022 & 0.020 & 0.810    & 0.744   \\ \hline
8  & IJCAIconf       & 8.154                  & 0.010 & 0.009 & 0.280    & 0.224   \\ \hline
9  & ACMUIST         & 79.134                 & 0.025 & 0.024 & 1.507    & 1.22    \\ \hline
10 & WSDMSocial      & 26.263                 & 0.035 & 0.029 & 0.982    & 0.921   \\ \hline
\end{tabular}
\end{table}
